Building your path to escape from home

Random walks on dynamic graphs have received increasingly more attention from different academic communities over the last decade. Despite the relatively large literature, little is known about random walks that construct the graph where they walk while moving around. In this paper we study one of the simplest conceivable discrete time models of this kind, which works as follows: before every walker step, with probability $p$ a new leaf is added to the vertex currently occupied by the walker. The model grows trees and we call it the Bernoulli Growth Random Walk (BGRW). We show that the BGRW walker is transient and has a well-defined linear speed $c(p)>0$ for any $0<p\leq 1$. We also show that the tree as seen by the walker converges (in a suitable sense) to a random tree that is one-ended. Some natural open problems about this tree and variants of our model are collected at the end of the paper.

==> averagelocalfunctions-revision.tex <==
%!TEX root = draft_reorganizar.tex

%The basic material in this section is covered in detail in \cite{AldousSteele_Objective,Bordenave2016}.
%This section is devoted to investigate the behavior of observables of the \textit{BGRW} that depend only of finite structures around the walker and exploit its consequences. The convergence of the average of such observables is closely related to a sort of \textit{loss of memory} of the \textit{BGRW} process, which will be better explained latter. For now, we are going to introduce the concepts of \textit{rooted graphs} and \textit{local functions} to properly define what is meant by ``finite structures around the walker" and state our results.



\ignore{\subsection{Loss of memory} 
\notarodrigo{Intuition on the loss of memory}

An important step in the proof of Theorem~\ref{thm:rfuncthm}
is to show that the initial condition does not affect the long time behavior of $\widehat{P}_n(\psi)$ (see, Lemma~\ref{lemma:indep}). The latter result relies on a sort of \textit{loss of memory} of the \textit{BGRW} process  which allows to compare the process starting from an arbitrary initial condition $(T_0,X_0)$ with a refreshed process starting from a simpler  initial condition $(L,r)$ which is chosen to be \textit{a path of length $r$, with the walker at its further tip} (see, Lemma~\ref{lemma:crucial}). The parameter $r$ will be chosen properly according to our needs.
 

In order to compare the \textit{BGRW} process starting from an arbitrary initial condition with the \textit{BGRW} starting from the condition $(L,r)$, we introduce the following stopping time
\begin{equation}
\tau_r := \inf \left \lbrace n \ge 0 \; \middle | \; [T_n,X_n]_r = [L,r]\right \rbrace
\end{equation}
in other words, $\tau_{r}$ is the first time the walker $X$ is at the further tip of a path of length $r$.

The following lemma tells us that in average the walker does not take too long to find itself at the further tip of $L$.

\begin{definition}Given $C>0$ and $\alpha>1$, we say that the initial distribution $\mu$ is $(C,\alpha)$-bounded if for all $n,k\geq 1$:
\begin{equation}\label{eq:condicaolegal}\frac{1}{n+1}\sum_{t=0}^n\Pd_{\mu}(d_t(X_t)\geq k)\leq \frac{C}{k^\alpha}.\end{equation}
\end{definition} 




\begin{lemma}\label{lemma:taur} Assume the initial distribution $\mu$ is $(C,\alpha)$-bounded as in (\ref{eq:condicaolegal}). Then for all $n\in\N$, $n\geq 1$:
	\begin{equation*}
\Ed_{T_0,x_0}[\tau_r\wedge n]\leq \left(C +\frac{r2^{r-1}}{p^r}\right)\,n^{\frac{2}{1+\alpha}}.\end{equation*}
\end{lemma}
\begin{proof} We begin with some notation. Given $\beta>0$ (to be chosen later), let $\eta_n$ be the first time the walker "sees" a node with degree $\geq n^\beta$.
	%	 
	\begin{equation}
	\eta_n := \inf \left \lbrace m \ge 0 \; \middle | \; d_{m}(X_m)\geq n^\beta\right \rbrace
	\end{equation}
	and consider the event $A_i$ in which at time $ir$ the walker creates a new leaf, jumps to it and grows a path of length $r-1$ from it in such way that at time $ir+r-1$ the walker finds itself at the tip of a path of length $r$. Now we define another stopping time
	\begin{equation}
	\tilde{\tau_r} := \inf \left \lbrace i \ge 0 \; \middle | \; A_i \text{ occurs }\right \rbrace
	\end{equation}
	and note that $\tau_r \le r\tilde{\tau_r}$.
	
	By the definition of the event $A_i$, we have that
	\[
	\Pd_{T_0,x_0} \left( A_i \middle | \mathcal{F}_{ir}\right) = \frac{p}{d_{ir}(X_{ir})}\left(\frac{p}{2}\right)^{r-1}.
	\]
	Thus, by the definition of the stopping time $\eta_n$, we also have
	\begin{equation}
	\mathbb{1}\{\eta_n > ir \}\Pd_{T_0,x_0} \left( A_i \middle | \mathcal{F}_{ir}\right) \ge \frac{p}{n^\beta}\left(\frac{p}{2}\right)^{r-1}\mathbb{1}\{\eta > ir \}.
	\end{equation}
	Using the above inequality and noticing that $\mathbb{1}\{\eta > kr\} \le \mathbb{1}\{\eta_n > (k-1)r\}$, we obtain
	\begin{equation}
	\begin{split}
	\Pd_{T_0,x_0}\left( \tilde{\tau_r} \ge k, \eta > kr\right) & = \Ed_{T_0,x_0} \left[ \Ed_{T_0,x_0} \left[ \mathbb{1}_{A^c_k} \middle | \mathcal{F}_{kr}\right]\mathbb{1}\{\eta > kr \} \prod_{i=0}^{k-1}\mathbb{1}_{A^c_i} \right] \\
	& \le \left(1- \frac{p}{n^\beta}\left(\frac{p}{2}\right)^{r-1}\right)\Pd_{T_0,x_0}\left( \tilde{\tau_r} \ge k-1, \eta > (k-1)r\right).
	\end{split}
	\end{equation}
	Then, proceeding by induction, we obtain the following upper bound
	\begin{equation}
	\Pd_{T_0,x_0}\left( \tilde{\tau_r} \ge k, \eta > kr\right) \le \left(1- \frac{p}{n^\beta}\left(\frac{p}{2}\right)^{r-1}\right)^k\leq \exp\left(-\frac{pk}{n^\beta}\left(\frac{p}{2}\right)^{r-1}\right).
	\end{equation}
	Since
	\[
	\Pd_{T_0,x_0}\left( \tau_r \wedge n \ge k \right) \le \left\{\begin{array}{ll}\Pd_{T_0,x_0}\left( \tilde{\tau_r} \ge k/r \right)\leq \exp\left(-\frac{pk}{rn^\beta}\left(\frac{p}{2}\right)^{r-1}\right), & k\leq n\\ 0, & \mbox{otherwise};\end{array}\right.
	\]
	we obtain: 
	\begin{equation}\label{eq:expttilde}
	\Ed_{T_0,x_0}\left[ \tau_r\wedge n \right] \le \frac{r2^{r-1}}{p^r}n^\beta + n\,\Pd_{T_0,x_0} \left( \eta_n \le n\right).
	\end{equation}
	But, by our condition (\ref{eq:condicaolegal}),
	\[\Pd_{T_0,x_0} \left( \eta_n \le n\right)\leq \sum_{t=0}^n\Pd_{T_0,x_0}(d_t(X_t)\geq n^\beta)\leq \frac{C}{n^{\alpha\beta-1}},\]
	so
	\[\Ed_{T_0,x_0}\left[ \tau_r\wedge n \right] \le \frac{r2^{r-1}}{p^r}n^\beta + C\,n^{2-\alpha\beta}.\]
	Since $\alpha>1$, we may choose 
	\[\beta:=\frac{2}{1+\alpha}\in(0,1)\]
	and obtain:
	\[\Ed_{T_0,x_0}\left[ \tau_r\wedge n \right] \le \left(C +\frac{r2^{r-1}}{p^r}\right)\,n^{\frac{2}{1+\alpha}}.\] 
	
	
	
\end{proof}
We point out that the above lemma and Markov's inequality imply that the stopping time~$\tau_{r}$ is finite almost surely for all fixed $r$.}

\subsection{Proof of the main theorem of the section}
{\color{red} to be continued....}
\begin{lemma}\label{lemma:indep}
	Given independent process BGRW started from $(T_0,x_0)$ and $(T_0',x_0')$, the limits of $\{\widehat{P}_n(\psi)\}_{n \in \N }$ are the same for the two processes.
\end{lemma}
\begin{proof}
	Let $\{\widehat{P}_n(\psi)\}_{n \in \N }$ and $\{\widehat{P'}_n(\psi)\}_{n \in \N }$ be as above for each one of the process. Also, let $A_n$ be the following event
	\begin{equation}\label{def:An}
	A_n := \left \lbrace \left| \widehat{P}_n(\psi) - \Ed_{L,2r} \left[ \widehat{P}_q(\psi)\right]\right| \ge \frac{1}{\log n} + err_n(r,q) \right \rbrace.
	\end{equation}
	Recall that, \textit{w.h.p}, both $\dmax{n}$ and $d_{\text{max}}(T'_n)$, are at most $\max\{\dmax{0}, d_{\text{max}}(T'_0) \}+ c \log n$. Using triangle inequality and assuming $r \sim \log n$ and $q \sim n^{\alpha}$, we obtain
	\begin{equation}
	\begin{split}
	\Pd \left( 	\left|\widehat{P}_n(\psi) - \widehat{P}_{n'}(\psi)\right| \ge \frac{2}{\log n} + 2err_n(r,q)\right) & \le \Pd \left( A_n \right) + \Pd \left( A'_n \right) \le c \exp \left \lbrace - \frac{n^{1-\alpha}}{C\log^{2\g}n} \right \rbrace.
	\end{split}
	\end{equation}
	Finally, by Borel-Cantelli Lemma we obtain that \textit{a.s.}
	\begin{equation}
	\left|\widehat{P}_n(\psi) - \widehat{P}_{n'}(\psi)\right| \le \frac{2}{\log n} + 2err_n(r,q)
	\end{equation}
	for large $n$. This implies that both sequences converges to the same limit.
\end{proof}


==> averagelocalfunctions.tex <==
%!TEX root = draft_reorganizar.tex

%The basic material in this section is covered in detail in \cite{AldousSteele_Objective,Bordenave2016}.
%This section is devoted to investigate the behavior of observables of the \textit{BGRW} that depend only of finite structures around the walker and exploit its consequences. The convergence of the average of such observables is closely related to a sort of \textit{loss of memory} of the \textit{BGRW} process, which will be better explained latter. For now, we are going to introduce the concepts of \textit{rooted graphs} and \textit{local functions} to properly define what is meant by ``finite structures around the walker" and state our results.


The main result of this section is about the empirical averages of \textit{local function} on the space $\sT_*$ along trajectories. Recall the definition of the empirical measure from Section \ref{sec:finiteinfinite}.

\begin{theorem}\label{thm:rfuncthm}For each parameter $0<p\leq 1$ and each bounded $r$-local function $\psi:\sT_*\to \R$, there exists a constant $\mathcal{M}(\psi)=\mathcal{M}_p(\psi)$ such that, for all initial conditions $(T_0,x_0)$,
\[\lim_{n\to +\infty}\widehat{P}_n(\psi) =\mathcal{M}(\psi)\mbox{ }\mathbb{P}_{T_0,x_0}\mbox{-a.s.}.\]
\end{theorem}
As we will see in the next section, this result implies that ``the tree seen by the walker"~converges to an infinite random tree when $n\to +\infty$.  


\subsection{Existence of the speed} Before we go to the proof of Theorem~\ref{thm:rfuncthm}, we prove, as an application of it, that the random walker in the \textit{BGRW} model has a speed and it is positive.
\begin{theorem}[Linear speed of the walker] There exists a positive constant $c$ depending on $p$ only, such that, for all initial condition $(T_0,x_0)$ we have
	\[
	\lim_{n\rightarrow \infty } \frac{d(X_n,root)}{n}  = c, \; \textit{a.s.}
	\]
\end{theorem}
\begin{proof} Recall that by Proposition~\ref{prop:liminf}, we already have
	\begin{equation}
	\liminf_{n \rightarrow \infty} \frac{d(X_n, \mathrm{root})}{n} = c >0, \; \textit{a.s.},
	\end{equation}
	for some positive constant $c$ depending on $p$ only. To extend the result to the actual limit, we prove that the distance from the root at time $n$ may be written as a martingale of order~$\sqrt{n\log n}$ plus a sum of $1$-local functions. First observe that
	\begin{equation}
	\begin{split}
	\mathbb{E}\left[ \Delta d(X_n, \mathrm{root}) \mid  \mathcal{F}_{n}\right]  
	%& =-\frac{p}{\deg_{T_n}X_n + 1} - \frac{(1-p)}{\deg_{T_n}X_n}+\frac{p\deg_{T_n}X_n}{\deg_{T_n}X_n + 1} + \frac{(1-p)(\deg_{T_n}X_n - 1)}{\deg_{T_n}X_n} \\
	& = \frac{p(\deg_{T_n}X_n-1)}{\deg_{T_n}X_n + 1} + \frac{(1-p)(\deg_{T_n}X_n - 2)}{\deg_{T_n}X_n}.
	\end{split}
	\end{equation}
	Thus, by Doob's Decomposition Theorem, we obtain
	\begin{equation}
	d(X_{n+1}, \mathrm{root}) = M_{n+1} + \sum_{j=1}^n \psi(T_j,X_j),
	\end{equation}
	where $M_{n+1}$ is a bounded increment martingale and $\psi$ is the $1$-local function defined as
	\[
	\psi(T_j,X_j) :=  \frac{p(\deg_{T_j}X_j-1)}{\deg_{T_j}X_j + 1} + \frac{(1-p)(\deg_{T_j}X_j - 2)}{\deg_{T_j}X_j}.
	\]
	Finally, Azuma's inequality gives us that $M_n$ is of order $\sqrt{n\log n}$, \textit{w.h.p} and Theorem \ref{thm:rfuncthm} gives us that 
	\[
	\lim_{n\rightarrow \infty }\frac{1}{n}\sum_{j=1}^n \psi(T_j,X_j) = c, \textit{a.s},
	\]
	where $c$ is a constant depending on $p$ and $\psi$ only. Combining these with (\ref{ineq:posliminf}) we finally prove that
	\[
	\lim_{n\rightarrow \infty } \frac{d(X_n, \mathrm{root})}{n} = c, \textit{a.s}
	\]
	where $c$ is a positive constant.
\end{proof}
\ignore{\subsection{Loss of memory} 
\notarodrigo{Intuition on the loss of memory}

An important step in the proof of Theorem~\ref{thm:rfuncthm}
is to show that the initial condition does not affect the long time behavior of $\widehat{P}_n(\psi)$ (see, Lemma~\ref{lemma:indep}). The latter result relies on a sort of \textit{loss of memory} of the \textit{BGRW} process  which allows to compare the process starting from an arbitrary initial condition $(T_0,X_0)$ with a refreshed process starting from a simpler  initial condition $(L,r)$ which is chosen to be \textit{a path of length $r$, with the walker at its further tip} (see, Lemma~\ref{lemma:crucial}). The parameter $r$ will be chosen properly according to our needs.
 

In order to compare the \textit{BGRW} process starting from an arbitrary initial condition with the \textit{BGRW} starting from the condition $(L,r)$, we introduce the following stopping time
\begin{equation}
\tau_r := \inf \left \lbrace n \ge 0 \; \middle | \; [T_n,X_n]_r = [L,r]\right \rbrace
\end{equation}
in other words, $\tau_{r}$ is the first time the walker $X$ is at the further tip of a path of length $r$.

The following lemma tells us that in average the walker does not take too long to find itself at the further tip of $L$.

\begin{definition}Given $C>0$ and $\alpha>1$, we say that the initial distribution $\mu$ is $(C,\alpha)$-bounded if for all $n,k\geq 1$:
\begin{equation}\label{eq:condicaolegal}\frac{1}{n+1}\sum_{t=0}^n\Pd_{\mu}(d_t(X_t)\geq k)\leq \frac{C}{k^\alpha}.\end{equation}
\end{definition} 




\begin{lemma}\label{lemma:taur} Assume the initial distribution $\mu$ is $(C,\alpha)$-bounded as in (\ref{eq:condicaolegal}). Then for all $n\in\N$, $n\geq 1$:
	\begin{equation*}
\Ed_{T_0,x_0}[\tau_r\wedge n]\leq \left(C +\frac{r2^{r-1}}{p^r}\right)\,n^{\frac{2}{1+\alpha}}.\end{equation*}
\end{lemma}
\begin{proof} We begin with some notation. Given $\beta>0$ (to be chosen later), let $\eta_n$ be the first time the walker "sees" a node with degree $\geq n^\beta$.
	%	 
	\begin{equation}
	\eta_n := \inf \left \lbrace m \ge 0 \; \middle | \; d_{m}(X_m)\geq n^\beta\right \rbrace
	\end{equation}
	and consider the event $A_i$ in which at time $ir$ the walker creates a new leaf, jumps to it and grows a path of length $r-1$ from it in such way that at time $ir+r-1$ the walker finds itself at the tip of a path of length $r$. Now we define another stopping time
	\begin{equation}
	\tilde{\tau_r} := \inf \left \lbrace i \ge 0 \; \middle | \; A_i \text{ occurs }\right \rbrace
	\end{equation}
	and note that $\tau_r \le r\tilde{\tau_r}$.
	
	By the definition of the event $A_i$, we have that
	\[
	\Pd_{T_0,x_0} \left( A_i \middle | \mathcal{F}_{ir}\right) = \frac{p}{d_{ir}(X_{ir})}\left(\frac{p}{2}\right)^{r-1}.
	\]
	Thus, by the definition of the stopping time $\eta_n$, we also have
	\begin{equation}
	\mathbb{1}\{\eta_n > ir \}\Pd_{T_0,x_0} \left( A_i \middle | \mathcal{F}_{ir}\right) \ge \frac{p}{n^\beta}\left(\frac{p}{2}\right)^{r-1}\mathbb{1}\{\eta > ir \}.
	\end{equation}
	Using the above inequality and noticing that $\mathbb{1}\{\eta > kr\} \le \mathbb{1}\{\eta_n > (k-1)r\}$, we obtain
	\begin{equation}
	\begin{split}
	\Pd_{T_0,x_0}\left( \tilde{\tau_r} \ge k, \eta > kr\right) & = \Ed_{T_0,x_0} \left[ \Ed_{T_0,x_0} \left[ \mathbb{1}_{A^c_k} \middle | \mathcal{F}_{kr}\right]\mathbb{1}\{\eta > kr \} \prod_{i=0}^{k-1}\mathbb{1}_{A^c_i} \right] \\
	& \le \left(1- \frac{p}{n^\beta}\left(\frac{p}{2}\right)^{r-1}\right)\Pd_{T_0,x_0}\left( \tilde{\tau_r} \ge k-1, \eta > (k-1)r\right).
	\end{split}
	\end{equation}
	Then, proceeding by induction, we obtain the following upper bound
	\begin{equation}
	\Pd_{T_0,x_0}\left( \tilde{\tau_r} \ge k, \eta > kr\right) \le \left(1- \frac{p}{n^\beta}\left(\frac{p}{2}\right)^{r-1}\right)^k\leq \exp\left(-\frac{pk}{n^\beta}\left(\frac{p}{2}\right)^{r-1}\right).
	\end{equation}
	Since
	\[
	\Pd_{T_0,x_0}\left( \tau_r \wedge n \ge k \right) \le \left\{\begin{array}{ll}\Pd_{T_0,x_0}\left( \tilde{\tau_r} \ge k/r \right)\leq \exp\left(-\frac{pk}{rn^\beta}\left(\frac{p}{2}\right)^{r-1}\right), & k\leq n\\ 0, & \mbox{otherwise};\end{array}\right.
	\]
	we obtain: 
	\begin{equation}\label{eq:expttilde}
	\Ed_{T_0,x_0}\left[ \tau_r\wedge n \right] \le \frac{r2^{r-1}}{p^r}n^\beta + n\,\Pd_{T_0,x_0} \left( \eta_n \le n\right).
	\end{equation}
	But, by our condition (\ref{eq:condicaolegal}),
	\[\Pd_{T_0,x_0} \left( \eta_n \le n\right)\leq \sum_{t=0}^n\Pd_{T_0,x_0}(d_t(X_t)\geq n^\beta)\leq \frac{C}{n^{\alpha\beta-1}},\]
	so
	\[\Ed_{T_0,x_0}\left[ \tau_r\wedge n \right] \le \frac{r2^{r-1}}{p^r}n^\beta + C\,n^{2-\alpha\beta}.\]
	Since $\alpha>1$, we may choose 
	\[\beta:=\frac{2}{1+\alpha}\in(0,1)\]
	and obtain:
	\[\Ed_{T_0,x_0}\left[ \tau_r\wedge n \right] \le \left(C +\frac{r2^{r-1}}{p^r}\right)\,n^{\frac{2}{1+\alpha}}.\] 
	
	
	
\end{proof}
We point out that the above lemma and Markov's inequality imply that the stopping time~$\tau_{r}$ is finite almost surely for all fixed $r$.}

The next lemma tells us that, in average, the empirical average $\widehat{P}_n(\psi)$ starting from an arbitrary initial condition $(T_0,x_0)$ is close to its counterpart starting from the initial condition~$(L,r)$.
Before stating the lemma, let us introduce the following quantities
\begin{equation}\label{def:alphar}
\alpha(r,n) := \Pd_{L,2r} \left( X \text{ visits middle point of } L \text{ before time } n\right)
\end{equation}
and 
\begin{equation}\label{def:alpharinf}
\alpha(r) := \Pd_{L,2r} \left( X \text{ visits middle point of } L \text{ in finite time}\right).
\end{equation}
%\begin{lemma}[Crucial Lemma]\label{lemma:crucial} Suppose $\psi$ is $r$-local, $(T_0,x_0)$ and $q \in \N$ are given. Also, let $U_q$ be uniform over $\{1,2,\cdots, q \}$ and independent of $(T_t,X_t)_{t=0}^q$ a \textit{BGRW} starting from $(T_0,x_0)$. Let $V_q$ be uniform over $\{ 0,1,\cdots, q\}$ and independent of $(T_t^{(2r)},X_t^{(2r)})$. Then,
%	\begin{equation}
%	\left | \Ed \left( \psi\left(T_{U_q},X_{U_q}\right)\right) - \Ed \left( \psi\left(T^{(2r)}_{V_q},X^{(2r)}_{V_q}\right)\right)\right | \le 2\alpha(r) + \frac{2\|\psi\|_{\infty}\Ed_{T_0,x_0}(\tau_{2r}\wedge q)}{q}.
%	\end{equation}
%\end{lemma}
\begin{lemma}[Crucial Lemma]\label{lemma:crucial} For all bounded $r$-local functions $\psi$ and all initial conditions~$(T_0,x_0)$, the following holds 
	\begin{equation}
	\left | \Ed_{T_0,x_0} \left[ \widehat{P}_n(\psi)\right] - \Ed_{L,2r} \left[ \widehat{P}_n(\psi)\right]\right | \le 2\alpha(r,n) + \frac{2\|\psi\|_{\infty}\Ed_{T_0,x_0}[\tau_{2r}\wedge (n+1)]}{n+1}.
	\end{equation}
\end{lemma}
\begin{proof}
	Let $\s_{2r}$ be the following stopping time
	\begin{equation*}
	\s_{2r} := \inf \left \lbrace t\ge 0 \; \middle | \; X_{t+\tau_{2r}} \text{ occupies the middle point of the } 2r\text{-path from time }\tau_{2r}\right \rbrace.
	\end{equation*}
	Since $\tau_{2r}$ is finite almost surely, $\sigma_{2r}$ is well-defined.
	
	Let $\{(T_t^{(2r)},X_t^{(2r)})\}_{t \ge 0}$ denote a \textit{BGRW} process starting from $(L,2r)$. Observe that one may couple the processes $\{(T_{t+\tau_{2r}},X_{t+\tau_{2r}})\}_{t\ge 0}$ and $\{(T_t^{(2r)},X_t^{(2r)})\}_{t \ge 0}$ in such way that their $r$-neighborhoods 
	are the same as rooted trees. More precisely, one may couple the two processes so that
	\[
	\left[T_{t+\tau_{2r}},X_{t+\tau_{2r}}\right]_{r}  = \left[T^{(2r)}_{t},X^{(2r)}_{t}\right]_{r},
	\]
	as long as $t\le\s_{2r}$. Since $\psi$ is $r$-local, this implies that
	\[
	\psi(T_{t+\tau_{2r}}, X_{t+\tau_{2r}}) = \psi(T_{t}^{(2r)}, X^{(2r)}_{t}),
	\]
	for all $t$ less than $\s_{2r}$. In particular,
	\begin{equation}
	\begin{split}
	\left| \frac{1}{n+1}\sum_{t=0}^n \left[\psi(T_{t+\tau_{2r}}, X_{t+\tau_{2r}}) - \psi(T_{t}^{(2r)}, X^{(2r)}_{t})\right]\right| & \le 2\|\psi\|_{\infty}\mathbb{1}\{\s_{2r}<n\}.
	\end{split}
	\end{equation}
	Thus
	\begin{equation}\label{eq:pstau}
	\left|\Ed_{T_0,x_0}\left[\frac{1}{n+1}\sum_{t=0}^n \psi(T_{t+\tau_{2r}}, X_{t+\tau_{2r}})\right] - \Ed_{L,2r}\left[\widehat{P}_n(\psi)\right]\right| \le 2\alpha(r,n),
	\end{equation}
	since the processes $\{(T_{t+\tau_{2r}},X_{t+\tau_{2r}})\}_{t\ge 0}$ and $\{(T_t^{(2r)},X_t^{(2r)})\}_{t \ge 0}$ are coupled until $\sigma_{2r}$, it follows that
	\begin{equation}
	\mathbb{P}_{T_0,x_0}(\sigma_{2r} < n) = \alpha(r,n).
	\end{equation}
	Using again that $\psi$ is bounded, the following bound holds deterministically
	\begin{equation}
	\begin{split}
	\left| \frac{1}{n+1}\sum_{t=0}^n\left[ \psi(T_{t}, X_{t}) - \psi(T_{t+\tau_{2r}}, X_{t+\tau_{2r}})\right]\right| & \le \frac{2\|\psi\|_{\infty}(\tau_{2r}\wedge (n+1))}{n+1}
	\end{split}
	\end{equation}
	and implies
	\begin{equation}\label{eq:psiuq}
	\left|\Ed_{T_0,x_0}\left[\widehat{P}_n(\psi)\right]-\Ed_{T_0,x_0}\left[\frac{1}{n+1}\sum_{t=0}^n \psi(T_{t+\tau_{2r}}, X_{t+\tau_{2r}})\right]\right| \le \frac{2\|\psi\|_{\infty}\Ed[\tau_{2r}\wedge (n+1)]}{n+1}.
	\end{equation}
	Finally, using (\ref{eq:pstau}) and (\ref{eq:psiuq}) and triangle inequality we prove the lemma.
\end{proof}
\subsection{Proof of the main theorem of the section}
%\begin{lemma}\label{lemma:ME}
%	Let $(T_0,x_0)$ and $\varepsilon >0$ be given. Assume $-1\le \psi \le 1$ is $r_0$-local. Then for any $r > r_0$, $q<n$ and $k = \lfloor n/q \rfloor$, there exists a positive constant $C$ depending on $p$ only such that the average
%	\[
%	M_n(\psi) := \frac{1}{n} \sum_{t=1}^n \psi \left(T_t,X_t\right)
%	\]
%	satisfies
%	\begin{equation}
%	\Pd_{T_0,x_0} \left( \left | M_n(\psi) - \Ed\left( \psi \left( T^{(2r)}_{V_q}, X^{(2r)}_{V_q}\right)\right) \right | \ge \varepsilon + err_n(q,r) \right) \le 4\exp\{ - \varepsilon^2k/32\},
%	\end{equation}
%	where 
%	\begin{equation}
%	err_n(q,r) := \frac{2q}{n} + 2\alpha(r) + \frac{2^{2r+1}r}{p^{2r}}\frac{(C\log(q)+\dmax{n})}{q} + \frac{4r|V(T_0)|}{q^9}+ \frac{4r+k}{q^8}. %\frac{4r\left(\frac{2}{p}\right)^{2r}}{k-1}\sum_{i=1}^{k}\frac{\Ed_{T_0,x_0}\left[\Delta(T_{(i+1)q})\middle | \mathcal{F}_{iq}\right]}{q}.
%	\end{equation}
%\end{lemma}
%\begin{proof}We begin by defining some notation. Let $g_t$ be $\psi(T_t,X_t)$, and denote by $\mathcal{G}_i$ the $\s$-algebra generated by the process $\{(T_t,X_t)\}_{t\in \N}$ up to time $iq$ and set
%	\begin{equation}
%	M_n(\psi) = \frac{1}{n}\sum_{t=1}^{n}g_t.
%	\end{equation}
%	By Lemma \ref{lemma:A}, if $U_i$ is uniform over $((i-1)q,iq] \cap \N$, we have
%	\begin{equation}
%	\Pd \left( \left|M_n(\psi) - \frac{1}{k}\sum_{i=1}^kg_{U_i} \right| \ge \e/2 + 2q/n \right) \le 2\exp\left \lbrace - \frac{\varepsilon^2k}{8} \right \rbrace.
%	\end{equation}
%	Moreover, the sequence 
%	\[
%	\{ (g_{U_i} - \Ed \left[g_{U_i} \middle | \mathcal{G}_{i-1}\right]), \mathcal{G}_i\}_{i=1}^k
%	\]
%	is a martingale difference sequence with increment lying on $[-2,2]$. Consequently, applying Azuma's inequality we obtain
%	\begin{equation}
%	\Pd \left( \left|\frac{1}{k}\sum_{i=1}^k\left(g_{U_i} - \Ed \left[g_{U_i} \middle | \mathcal{G}_{i-1}\right] \right) \right| \ge \e/2 \right) \le 2\exp\left \lbrace - \frac{\varepsilon^2k}{32} \right \rbrace.
%	\end{equation}
%	We now show that the inequality below holds deterministically.
%	\begin{equation}\label{eq:eu}
%	\begin{split}
%	\left| \Ed \left[g_{U_{i+1}} \middle | \mathcal{G}_{i}\right] - \Ed \left[\psi\left(T^{(2r)}_{V_q},X^{(2r)}_{V_q}\right)\right]\right| & \le 2\alpha(r)+ \frac{2^{2r+1}r}{p^{2r}}\frac{(C\log(q)+\dmax{n})}{q} \\
%	&  \hspace{0.5cm}+ \frac{4r(|V(T_0)|+iq)}{q^9} + \frac{4r}{q^8}.
%	\end{split}
%	\end{equation}
%	This implies the theorem using triangle inequality. To see this, note that since the random variable~$U_i = iq + \tilde{U}_q$, where $\tilde{U}_q$ is uniform on $\{1,2,\cdots,q\}$, the Markov property, shifting the chain at time $iq$, gives us
%	\begin{equation}
%	\Ed \left[ g_{U_{i+1}} \middle| \mathcal{G}_{i} \right] = \Ed_{T_{iq},X_{iq}} \left[\psi\left(T_{\tilde{U}_q}, X_{\tilde{U}_q}\right)\right].
%	\end{equation}
%	Then, by Lemma \ref{lemma:crucial} we have
%	\begin{equation}
%	\begin{split}
%	\left| \Ed_{T_{iq},X_{iq}} \left[\psi\left(T_{\tilde{U}_q}, X_{\tilde{U}_q}\right)\right] - \Ed \left[\psi\left(T^{(2r)}_{V_q},X^{(2r)}_{V_q}\right)\right]\right| & \le 2\alpha(r) + \frac{2\Ed_{T_{iq},X_{iq}}(\tau_{2r}\wedge q)}{q}
%	\end{split}
%	\end{equation}
%	and by Lemma \ref{lemma:taur} we also have
%	\begin{equation}
%	\Ed_{T_{iq},X_{iq}}(\tau_{2r}\wedge q) \le \frac{2^{2r+1}r}{p^{2r}}(C\log q + \dmax{n}) + \frac{4r|V(T_{0})|+iq}{q^{8}} + \frac{4r}{q^{7}},
%	\end{equation}
%	since both $|V(T_{iq})| \le |V(T_{0})|+iq$ and the maximum degree is increasing on the time deterministically.
%	
%	To simplify our writing, let $\beta(i,q,r)$ be the following function
%	\begin{equation}
%	\beta(i,q,r) :=  2\alpha(r)+ \frac{2^{2r+1}r}{p^{2r}}\frac{(C\log(q)+\dmax{n})}{q} + \frac{4r(|V(T_0)|+iq)}{q^9} + \frac{4r}{q^8}.
%	\end{equation}
%	Then
%	\begin{equation}
%	\frac{1}{k}\sum_{i=1}^{k}\beta(i,q,r) \le 2\alpha(r)+ \frac{2^{2r+1}r}{p^{2r}}\frac{(C\log(q)+\dmax{n})}{q} + \frac{4r|V(T_0)|}{q^9}+ \frac{4r+k}{q^8}.
%	\end{equation}
%	Finally, using triangle inequality and (\ref{eq:eu}) we obtain deterministically
%	\begin{equation}\label{eq:eus}
%	\left| \frac{1}{k}\sum_{i=1}^{k}\left(\Ed \left[g_{U_{i+1}} \middle | \mathcal{G}_{i}\right]\right) - \Ed \left[\psi\left(T^{(2r)}_{V_q},X^{(2r)}_{V_q}\right)\right]\right| \le \frac{1}{k}\sum_{i=1}^{k}\beta(i,q,r).
%	\end{equation}
%	Combining the above with triangle inequality we prove the lemma.
%\end{proof}
\begin{lemma}\label{lemma:ME}
	Let $(T_0,x_0)$ and $\varepsilon >0$ be given. Assume $-1\le \psi \le 1$ is $r_0$-local. Then for any $r > r_0$, $q<n$ and $k = \lfloor n/q \rfloor$, there exists a positive constant $C$ depending on $p$ only such that
	\begin{equation}
	\Pd_{T_0,x_0} \left( \left | \widehat{P}_n(\psi) - \Ed_{L,2r}\left[ \widehat{P}_q(\psi) \right] \right | \ge \varepsilon + err_n(q,r) \right) \le 4\exp\{ - \varepsilon^2k/32\},
	\end{equation}
	where 
	\begin{equation}
	err_n(q,r) := \frac{2q}{n} + 2\alpha(r,q) + \frac{2^{2r+1}r}{p^{2r}}\frac{(C\log(q)+\dmax{n})}{q} + \frac{4r|V(T_0)|}{q^9}+ \frac{4r+k}{q^8}. %\frac{4r\left(\frac{2}{p}\right)^{2r}}{k-1}\sum_{i=1}^{k}\frac{\Ed_{T_0,x_0}\left[\Delta(T_{(i+1)q})\middle | \mathcal{F}_{iq}\right]}{q}.
	\end{equation}
\end{lemma}
\begin{proof}We begin by showing that it is enough to prove the result for $n=kq$. Write $n = kq+s$ and observe that the following deterministic bound holds
	\begin{equation*}
		\begin{split}
			\left | \frac{1}{n}\sum_{i=0}^{n-1}\psi(T_i,X_i) - \frac{1}{kq}\sum_{i=0}^{kq-1}\psi(T_i,X_i)\right | & = \left | \left(\frac{kq}{n}-1\right)\frac{1}{kq}\sum_{i=0}^{kq-1}\psi(T_i,X_i) + \frac{1}{n}\sum_{i=kq}^{kq+s-1}\psi(T_i,X_i)\right | \\
			& \le \frac{2 \|\psi \|_{\infty}s}{n} < \frac{2q}{n},
		\end{split}
	\end{equation*}
	since, by hypothesis, $\|\psi \|_{\infty} \le 1$. Then, we arrange~$\widehat{P}_{kq}(\psi)$ as follows
	\begin{equation}
	\begin{split}
	\widehat{P}_{kq}(\psi)= \frac{1}{kq}\sum_{i=0}^{kq-1}\psi(T_i,X_i) = \frac{1}{k}\left(\frac{1}{q}\sum_{i=0}^{q-1}\psi(T_i,X_i) + \cdots + \frac{1}{q}\sum_{i=kq-q}^{kq-1}\psi(T_i,X_i)\right)
	\end{split}
	\end{equation}
and, for $j \in \{1, \cdots, k\}$ let $S_j$ be the average
\begin{equation}\label{def:Sj}
S_j := \frac{1}{q}\sum_{i=(j-1)q}^{jq-1}\psi(T_i,X_i).
\end{equation}
Also, in order to simplify our writing, we denote by $\{\tilde{\mathcal{F}}_j\}_{j \ge 0}$ the following filtration
\begin{equation}
\tilde{\mathcal{F}}_0 = \mathcal{F}_0; \; \; \tilde{\mathcal{F}}_j = \mathcal{F}_{jq-1}.
\end{equation}
In this setup, by the definition of $S_j$, the process $\{S_j\}_{j \ge 1}$ is adapted to the filtration~$\{\tilde{\mathcal{F}}_j\}_{j \ge 0}$. Moreover, the process $\{M_k\}_{k \ge 1}$ defined as
\begin{equation}
M_k := \sum_{j=1}^{k} S_j - \Ed_{T_0,x_0}\left[ S_j \middle | \tilde{\mathcal{F}}_{j-1}\right] = M_{k-1} + S_k - \Ed_{T_0,x_0}\left[ S_k \middle | \tilde{\mathcal{F}}_{k-1}\right]
\end{equation}
is a mean zero martingale with respect to $\{\tilde{\mathcal{F}}_j\}_{j \ge 0}$ whose increments are bounded by $2$, since~$S_j$ is an average of random variables bounded by $1$. It will be useful to see $M_k$ as the following difference
\begin{equation}
M_k = k\widehat{P}_{kq}(\psi)  -\sum_{j=1}^k\Ed_{T_0,x_0}\left[ S_j \middle | \tilde{\mathcal{F}}_{j-1}\right].
\end{equation}
With all these definitions, by triangle inequality, we have that
\begin{equation}\label{ineq:triangle}
\begin{split}
	\left | \widehat{P}_n(\psi) - \Ed_{L,2r}\left[ \widehat{P}_q(\psi) \right] \right | & \le \frac{2q}{n} + \left|\frac{M_k}{k} \right| + \left|\frac{1}{k}\sum_{j=1}^k\left(\Ed_{T_0,x_0}\left[ S_j \middle | \tilde{\mathcal{F}}_{j-1}\right]-\Ed_{L,2r}\left[ \widehat{P}_q(\psi) \right]\right)\right|.
\end{split}
\end{equation}
To bound $M_k$ we apply Azuma's inequality which gives us
\begin{equation}\label{eq:Mk}
\Pd_{T_0,x_0}\left( \left|M_k\right| \ge \frac{\varepsilon k}{2}\right) \le 2\exp\{ - \varepsilon^2k/32\}.
\end{equation}
To bound the last term of the RHS of (\ref{ineq:triangle}), we first observe that by the Simple Markov Property, we have, for all $j \in \{1, \cdots, k\}$, the identity below
\begin{equation}
\Ed_{T_0,x_0}\left[ S_j \middle | \tilde{\mathcal{F}}_{j-1}\right] = \frac{1}{q}\sum_{i=1}^{q}\Ed_{T_{(j-1)q-1},X_{(j-1)q-1}} \left[ \psi(T_i,X_i)\right] = \Ed_{T_{(j-1)q-1},X_{(j-1)q-1}} \left[ \widehat{P}_q(\psi)\right].
\end{equation}
	Then, by Lemma \ref{lemma:crucial} we have
	\begin{equation}\label{ineq:SMQ}
	\begin{split}
	\left| \Ed_{T_0,x_0}\left[ S_j \middle | \tilde{\mathcal{F}}_{j-1}\right] - \Ed_{L,2r}\left[ \widehat{P}_q(\psi) \right]\right| & \le 2\alpha(r,q) + \frac{2\Ed_{T_{(j-1)q-1},X_{(j-1)q-1}} \left[\tau_{2r}\wedge q\right]}{q}
	\end{split}
	\end{equation}
	and by Lemma \ref{lemma:taur} we also have
	\begin{equation}
	\Ed_{T_{(j-1)q-1},X_{(j-1)q-1}} \left[\tau_{2r}\wedge q\right] \le \frac{2^{2r+1}r}{p^{2r}}(C\log q + \dmax{n}) + \frac{4r|V(T_{0})|+(j-1)q}{q^{8}} + \frac{4r}{q^{7}},
	\end{equation}
	since $|V(T_{(j-1)q})| \le |V(T_{0})|+(j-1)q$ and the maximum degree is deterministically increasing on the time.
	
	To simplify our writing, let $\beta(j,q,r)$ be the following function
	\begin{equation}
	\beta(j,q,r) :=  2\alpha(r,q)+ \frac{2^{2r+1}r}{p^{2r}}\frac{(C\log(q)+\dmax{n})}{q} + \frac{4r(|V(T_0)|+(j-1)q)}{q^9} + \frac{4r}{q^8}.
	\end{equation}
	Then
	\begin{equation}
	\frac{1}{k}\sum_{j=1}^{k}\beta(j,q,r) \le 2\alpha(r,q)+ \frac{2^{2r+1}r}{p^{2r}}\frac{(C\log(q)+\dmax{n})}{q} + \frac{4r|V(T_0)|}{q^9}+ \frac{4r+k}{q^8},
	\end{equation}
	which completes the proof.
\end{proof}
\begin{corollary} Let $\psi$ be a $r_0$-local function on $[-1,1]$, then $\{M_n(\psi)\}_{n\in \N}$ is a.s. a Cauchy sequence.
\end{corollary}
\begin{proof} The proof is essentially the claim below
	\begin{claim} For large enough $n$, there exist positive constants $c_0,c_1$ and $c_2$ depending on the parameter~$p$ and on the initial quantities $\dmax{0}$ and~$|V(T_0)|$ such that
		\begin{equation}
		\Pd_{T_0,x_0}\left( \left| \widehat{P}_m(\psi) - \widehat{P}_{m'}(\psi)\right|>\frac{c_0}{n^{c_1}}, \text{ for some }m,m'\in \{n,n+1,\cdots,n^2\}\right) \le \frac{c_2}{n^{4}}.
		\end{equation}
	\end{claim}
	\begin{claimproof}
		Let $q,r$ and $\e$ be
		\begin{equation}
		q= n^{1/3}\text{; } r= \left \lceil \frac{\log n}{12\log(2/p)} \right \rceil \text{ and } \e = n^{-1/6}.
		\end{equation}
		And recall that Proposition~\ref{prop:maxdeg} assures us the existence of a positive constant $c_4$ depending on $p$ only such that
		\begin{equation}\label{eq:probdmax}
		\Pd_{T_0,x_0} \left( \dmax{n^2} \ge \dmax{0}+ 10c_4^{-1}\log n \right) \le (|V(T_0)|+n^2) e^{-10\log n} \le \frac{c_5}{n^8},
		\end{equation}
		where $c_5$ is a positive constant depending on $|V(T_0)|$. Now, observe that for these choices, Lemma \ref{lemma:returntime} gives us
		\begin{equation}
		\alpha(r) \le e^{-c_6r} = \frac{1}{n^{c_7}}
		\end{equation}
		where $c_7$ depends on $p$ only. Moreover, for all $m \in \{n,n+1,\cdots,n^2\}$
		\begin{equation}\label{eq:bounderr}
		\begin{split}
		err_m(q,r) & = \frac{2q}{m} + 2\alpha(r) + \frac{2^{2r+1}r}{p^{2r}}\frac{(C\log(q)+\dmax{m})}{q} + \frac{4r|V(T_0)|}{q^9}+ \frac{4r+m/q}{q^8} \\
		& \le \frac{2}{n^{2/3}}+\frac{2}{n^{c_7}}+ \frac{c_8n^{1/6}\log n}{n^{1/3}} + \frac{c_9\log n}{n^{3}}+ \frac{c_{10}n^2}{n^{8/3}} \\
		& \le \frac{c_{11}}{n^{c_7}},
		\end{split}
		\end{equation}
		assuming $c_7 < 1/6$ and as long as $\dmax{n^2} \le \dmax{0}+ 10c_4^{-1}\log n$, which, by (\ref{eq:probdmax}), occurs with probability at least $1-c_5n^{-8}$.
		
		Now, by Lemma~\ref{lemma:ME}, for all $m \in \{n,n+1,\cdots,n^2\}$, we have
		\begin{equation}\label{eq:me2}
		\Pd_{T_0,x_0} \left( \left | \widehat{P}_m(\psi) - \Ed_{L,2r}\left[ \widehat{P}_q(\psi)\right] \right | \ge \varepsilon + err_m(q,r) \right) \le 4e^{ - c_{12}\varepsilon^2m/q} \le e^{-c_{13}n^{1/3}}.
		\end{equation}
		Combining the above bound with (\ref{eq:bounderr}) and using triangle inequality we obtain that
		\begin{equation}
		\Pd_{T_0,x_0} \left( \left | \widehat{P}_m(\psi) - \widehat{P}_{m'}(\psi) \right | \ge \frac{2c_{11}}{n^{c_7}}, \dmax{n^2} \le \dmax{0}+ 10c_4^{-1}\log n \right) \le 2e^{-c_{13}n^{1/3}}.
		\end{equation}
		Combining the above inequality with (\ref{eq:probdmax}) we obtain
		\begin{equation}
		\Pd_{T_0,x_0} \left( \left | \widehat{P}_m(\psi) - \widehat{P}_{m'}(\psi) \right | \ge \frac{2c_{11}}{n^{c_7}} \right) \le \frac{2c_5}{n^8}
		\end{equation}
		and finally, by union bound, we proof the claim.
	\end{claimproof}
	
	By the above claim and the first Borel-Cantelli lemma follows that almost surely there exist~$n_0$ such that, for all $m,m' \in \{n,n+1, \cdots, n^2\}$ with $n \ge n_0$ we have
	\[
	\left | \widehat{P}_m(\psi) - \widehat{P}_{m'}(\psi) \right | \le \frac{c_0}{n^{c_2}}.
	\]
	Given $\delta >0$, choose $n_1$ large enough so that $c_0/n_1^{c_2} < \delta$ and $n_1 \ge n_0$. Now, for $m, m' \ge n_1$ observe that, assuming $m \le m'$, there exists $k_0$ such that $m' \in \{m^{2^{k_0}},\cdots, m^{2{k_0+1}}\}$. Thus, 
	\begin{equation}
	\begin{split}
	\left | \widehat{P}_m(\psi) - \widehat{P}_{m'}(\psi) \right | & \le \sum_{j=1}^{k_0} \left | \widehat{P}_{m^{2^j}}(\psi) - \widehat{P}_{m^{2^{j+1}}}(\psi) \right | + \left | \widehat{P}_{m^{2k_0}}(\psi) - \widehat{P}_{m'}(\psi) \right | \\ 
	& \le \sum_{j=0}^{k_0}\frac{c_0}{(m^{2^j})^{c_2}} \le \frac{c_0}{m^{c_2}-1} \\
	& \le \frac{c_0}{n_1} < \delta,
	\end{split}
	\end{equation}
	which proves the corollary.
\end{proof}
\begin{lemma}\label{lemma:indep}
	Given independent process BGRW started from $(T_0,x_0)$ and $(T_0',x_0')$, the limits of $\widehat{P}_n(\psi)$ are the same for the two processes.
\end{lemma}
\begin{proof}
	Let $\widehat{P}_n(\psi)$ and $\widehat{P}'_n(\psi)$ be as above for each one of the process. Also, let $A_n$ be the following event
	\begin{equation}\label{def:An}
	A_n := \left \lbrace \left| \widehat{P}_n(\psi) - \Ed_{L,2r} \left[ \widehat{P}_q(\psi)\right]\right| \ge \frac{1}{\log n} + err_n(r,q) \right \rbrace.
	\end{equation}
	Recall that, \textit{w.h.p}, both $\dmax{n}$ and $d_{\text{max}}(T'_n)$, are at most $\max\{\dmax{0}, d_{\text{max}}(T'_0) \}+ c \log n$. Using triangle inequality and assuming $r \sim \log n$ and $q \sim n^{\alpha}$, we obtain
	\begin{equation}
	\begin{split}
	\Pd \left( 	\left|\widehat{P}_n(\psi) - \widehat{P}_{n'}(\psi)\right| \ge \frac{2}{\log n} + 2err_n(r,q)\right) & \le \Pd \left( A_n \right) + \Pd \left( A'_n \right) \le c \exp \left \lbrace - \frac{n^{1-\alpha}}{C\log^{2\g}n} \right \rbrace.
	\end{split}
	\end{equation}
	Finally, by Borel-Cantelli Lemma we obtain that \textit{a.s.}
	\begin{equation}
	\left|\widehat{P}_n(\psi) - \widehat{P}_{n'}(\psi)\right| \le \frac{2}{\log n} + 2err_n(r,q)
	\end{equation}
	for large $n$. This implies that both sequences converges to the same limit.
\end{proof}
\begin{proof}[Proof of Theorem~\ref{thm:rfuncthm}]
	Let $\{(T_n,X_n)\}_{n \in \N}$ and $\{(T'_n,X'_n)\}_{n \in \N}$ be two independent \textit{BGRW} processes starting from $(T_0,x_0)$ and $(T'_0,x'_0)$, respectively. Then, applying Lemma \ref{lemma:indep}, the respective $\{\widehat{P}_n(\psi)\}_{n \in \N}$ and $\{\widehat{P}'_n(\psi)\}_{n \in \N}$ processes converge to the same limit $\widehat{P}(\psi)$. Since the \textit{BGRW} processes are independent, the events $\{\widehat{P}(\psi) \in A\}$ and~$\{\widehat{P}(\psi) \in B\}$ are independents for all Borel sets on the real line. This implies that $\widehat{P}(\psi)$ is independent of itself, thus, constant almost surely.
\end{proof}

==> escape.tex <==
%!TEX root = draft_reorganizar.tex

\ignore{The convergence of empirical measures is related to the mixing properties of our process. In this section we present the main mechanism behind mixing. 

To do this, we first define certain stopping times. Given $\ell\in\N\backslash\{0\}$, let $P_\ell$ be the path of length $\ell$, ie. the graph with vertex set $\{0,1,\dots,\ell\}$ and edges $\{(i-1),i\}$ ($1\leq i\leq \ell$). We define $\tau_\ell$ as the first time when the graph around $X_t$ in $T_t$ is $P_\ell$.
\[\tau_\ell :=\inf\{t\geq 0\,:\, [T_t,X_t]_\ell = [P_\ell,\ell]\}.\]

\begin{definition}A measure $\mu$ over pairs $(T,x)$ is called $p$-escapable if $\tau_{\ell}<+\infty$ $\Pd_{\mu,p}$-almost surely for every $\ell\geq 1$.\end{definition} 

Not all trees are $p$-escapable. The next example gives a useful example to keep in mind.

\begin{example}[A hard tree]\label{ex:hardtree}Consider an infinite rooted tree $T_{\rm hard}$, with a root node $x_{\rm hard}$, such that each node at distance $h$ from the root has $g(h)>0$ children, with $1/g(h)$ summable. Consider the BGRW from $(T_{\rm hard},x_{\rm hard})$. One can show via the Borel-Cantelli Lemma that there is a positive probability that ${\rm dist}_{T_t}(X_t,x_{\rm hard}) = t$ for all $t\in\N$ (i.e. the walker simply ``walks down the tree"~for eternity). For the same reason, for any $\ell\in\N\backslash\{0\}$ there is a positive probability that $\tau_{\ell}=+\infty$. \end{example}

The next Lemmas (proven subsequently) explain why this concept is important to us. The first Lemma gives a quantitative criterion for ``escapability". In a way, it says that what makes the tree in Example \ref{ex:hardtree} non-escapable is that $X_t$ sees very large degrees along the way. 

\begin{lemma}[Quantitative escapability; proof in \S \ref{sec:proof.quantitative}]\label{lem:quantitative} Assume $\mu$ is a starting measure for which there exist $C,D,\alpha>0$ such that, for all $n,k\geq 1$,
\begin{equation}\label{eq:condicaolegal1}\sum_{t=0}^n\Pd_{\mu,p}(d_{T_t}(X_t)\geq k)\leq C\,(n+D)\,e^{-\alpha\,k}.\end{equation}
Then $\mu$ is $p$-escapable and
\begin{equation}\label{eq:estimateescapemu}\Ed_{\mu,p}(\tau_\ell\wedge n)\leq \frac{\ell 2^{\ell-1}}{p^\ell}\left\lceil \frac{2\log(n+D) + \log C}{\alpha}\right\rceil + 1.\end{equation}
Moreover, the following event holds with probability $\geq 1 - 1/n^{4}$: for all times $1\leq t\leq n$,  
\begin{equation}\label{eq:estimateescapefinite}\Ed_{T_t,X_t,p}(\tau_\ell\wedge n)\leq \frac{\ell 2^{\ell-1}}{p^\ell} \left\lceil \frac{\log(2n+D) +5\log n + \log C}{\alpha}\right\rceil + 1.\end{equation}
In particular, all measures $\mu=\delta_{(T,x)}$ with $T$ finite satisfy the above inequalities, with $C\leq e^{\alpha\,\Delta(T)}$ by virtue of Lemma \ref{lem:degreetail}.\end{lemma}
So Lemma \ref{lem:quantitative} also guarantees that not only $\mu$ is $p$-escapable, but also that, with high, each intermediate $T_t,X_t$ satisfies a quantitative escapability property. One important point is that the assumptions of Lemma \ref{lem:degreetail} always apply to initial trees that are finite, by virtue of Lemma \ref{lem:degreetail}.

\ignore{The second Lemma shows that the empirical measures of processes started from two $p$-escapable measures are asymptotically the same; ie. the initial distribution is ``forgotten". 

\begin{lemma}[Forgetfulness of empirical measures; proof in \S \ref{sec:proof.forget}]\label{lem:forget} Let $\mu$, $\nu$ be two $p$-escapable measures. Let $r>0$ and $\psi:\sT_*\to\R$ be a bounded $r$-local function. If there exists a constant $\mathcal{M}_p(\psi)$ such that $\widehat{P}_n\psi\to \mathcal{M}_p(\psi)$ $\Pd_{\nu,p}$-almost-surely, then we also have $\widehat{P}_n\psi\to \mathcal{M}_p(\psi)$ $\Pd_{\mu,p}$-almost-surely.
\end{lemma}}

Combining these results, we immediately obtain that, if we show that $\widehat{P}_n\psi$ converges for all $\nu=\delta_{(T_0,x_0)}$ supported on a single finite tree, the same property must hold (with the same limit) for all $p$-escapable initial measures. This greatly reduces the ammount of work in our proofs. 

\subsection{Quantitative escapability}\label{sec:proof.quantitative}
We prove here Lemma \ref{lem:quantitative}.

\begin{proof}[Proof of Lemma \ref{lem:quantitative}] We first prove inequality (\ref{eq:estimateescapemu}) for $\Ed_{\mu,p}(\tau_\ell\wedge n)$, noting that it implies $p$-escapability because, assuming it, we can show:
\[\Pd_{\mu,p}(\tau_{\ell}=+\infty)\leq \frac{\Ed_{\mu,p}(\tau_\ell\wedge n)}{n}\leq \frac{1}{n}\left(\frac{\ell 2^{\ell-1}}{p^\ell}\left\lceil \frac{2\log(n+D) + \log C}{\alpha}\right\rceil + 1\right)\stackrel{n\to +\infty}{\to} 0,\]
Fix some $\Delta>0$. Let $\eta_\Delta$ be the first time the walker "sees" a node with degree $\geq \Delta$.
	%	 
	\begin{equation}
	\eta_\Delta := \inf \left \lbrace m \ge 0 \; \middle | \; d_{m}(X_m)\geq \Delta\right \rbrace
	\end{equation}
	and consider the event $A_i$ in which at time $i\ell$ the walker creates a new leaf, jumps to it and grows a path of length $r-1$ from it in such way that at time $i\ell+\ell-1$ the walker finds itself at the tip of a path of length $\ell$. Now we define another stopping time
	\begin{equation}
	\tilde{\tau_\ell} := \inf \left \lbrace i \ge 0 \; \middle | \; A_i \text{ occurs }\right \rbrace
	\end{equation}
	and note that $\tau_\ell \le \ell\tilde{\tau_\ell}$.
	
	By the definition of the event $A_i$, we have that
	\[
	\Pd_{\mu,p} \left( A_i \middle | \mathcal{F}_{i\ell}\right) = \frac{p}{d_{i\ell}(X_{i\ell})}\left(\frac{p}{2}\right)^{\ell-1}.
	\]
	Thus, by the definition of the stopping time $\eta_\Delta$, we also have
	\begin{equation}
	\mathbb{1}\{\eta_\Delta > i\ell \}\Pd_{\mu,p} \left( A_i \middle | \mathcal{F}_{i\ell}\right) \ge \frac{p}{\Delta}\left(\frac{p}{2}\right)^{\ell-1}\mathbb{1}\{\eta_\Delta > i\ell \}.
	\end{equation}
	Using the above inequality and noticing that $\mathbb{1}\{\eta_\Delta > k\ell\} \le \mathbb{1}\{\eta_\Delta > (k-1)\ell\}$, we obtain
	\begin{equation}
	\begin{split}
	\Pd_{\mu,p}\left( \tilde{\tau_\ell} \ge k, \eta_\Delta > k\ell\right) & = \Ed_{\mu,p} \left[ \Ed_{\mu,p} \left[ \mathbb{1}_{A^c_k} \middle | \mathcal{F}_{k\ell}\right]\mathbb{1}\{\eta_\Delta > k\ell \} \prod_{i=0}^{k-1}\mathbb{1}_{A^c_i} \right] \\
	& \le \left(1- \frac{p}{\Delta}\left(\frac{p}{2}\right)^{\ell-1}\right)\Pd_{\mu,p}\left( \tilde{\tau_\ell} \ge k-1, \eta_\Delta > (k-1)\ell\right).
	\end{split}
	\end{equation}
	Then, proceeding by induction, we obtain the following upper bound
	\begin{equation}
	\Pd_{\mu,p}\left( \tilde{\tau_\ell} \ge k, \eta_\Delta > k\ell\right) \le \left(1- \frac{p}{\Delta}\left(\frac{p}{2}\right)^{\ell-1}\right)^k.
%	\leq \exp\left(-\frac{pk}{\Delta}\left(\frac{p}{2}\right)^{\ell-1}\right)
	\end{equation}
	Since
	\[
	\Pd_{\mu,p}\left( \tau_\ell \wedge n \ge k \ell \right) \le \left\{\begin{array}{ll}\Pd_{\mu,p}\left( \tilde{\tau_\ell} \ge k \right),
%	\leq \exp\left(-\frac{pk}{\ell\Delta}\left(\frac{p}{2}\right)^{\ell-1}\right),
	 & k\ell\leq n\\ 0, & \mbox{otherwise};\end{array}\right.
	\]
we have: 
	\begin{align*}
	\Pd_{\mu,p}\left( \tau_\ell \wedge n \ge k\ell \right) \leq \Pd_{\mu,p}\left(\tilde{\tau_\ell} \ge k ,\eta_\Delta>k\ell\right) + \Pd_{\mu,p}\left(\eta_\Delta\leq k\ell\right) ,
	\end{align*}
and consequently,
	\begin{equation}\label{eq:expttilde}
	\Ed_{\mu,p}\left[ \tau_\ell\wedge n \right] \le
	\sum_{j=0}^{\lfloor \frac{n}{\ell}\rfloor}
	\ell\Pd_{\mu,p}\left( \tau_\ell \wedge n \ge j \,r \right)
	\le \frac{\ell\,2^{\ell-1}}{p^\ell}\Delta + n\,\Pd_{\mu,p} \left( \eta_\Delta \le n\right).
	\end{equation}
	But, by our condition (\ref{eq:condicaolegal}),
	\begin{equation}\label{eq:conditionused}\Pd_{\mu,p} \left( \eta_\Delta \le n\right)\leq \sum_{t=0}^n\Pd_{\mu,p}(d_t(X_t)\geq \Delta)\leq C\,(n+1)\,e^{-\alpha\,\Delta}.\end{equation}
	so
	\[\Ed_{\mu,p}\left[ \tau_\ell\wedge n \right] \le \frac{\ell 2^{\ell-1}}{p^\ell}\Delta + C\,(n+1)^{2}e^{-\alpha\,\Delta}.\]
	We may choose \[\Delta = \left\lceil \frac{2\log (n+1) + \log C}{\alpha}\right\rceil\] to finish the proof of (\ref{eq:estimateescapemu}). 
	
	To prove the last statement in the Theorem, we go back to (\ref{eq:conditionused}) and note that was the only step in that proof where we used (\ref{eq:condicaolegal1}). In particular, we can go back to (\ref{eq:expttilde}) and obtain:
	\[\Ed_{T_t,X_t,p}\left[ \tau_\ell\wedge n \right] \le \frac{\ell 2^{\ell-1}}{p^\ell}\Delta + n\,\Pd_{T_t,X_t,p}(\eta_\Delta\leq n).\]
	In particular, if $\Delta$ is given and we consider the event  
	\[\mathcal{G}(\Delta):= \bigcap_{t=0}^n\{\Pd_{T_t,X_t,p}(\eta_\Delta\leq n)\leq 1/n)\},\]
	we have that, when $\mathcal{G}(\Delta)$ holds, then:
	\begin{equation}\label{eq:withoutcondition}\Ed_{T_t,X_t,p}(\tau_\ell\wedge n)\leq \frac{\ell 2^{\ell-1}}{p^\ell}\Delta + 1.\end{equation}
	for each $0\leq t\leq n$.
	To finish, we show that $\Pd_{\mu,p}(\mathcal{G}(\Delta))\geq 1 - n^{-4}$ for an appropriate choice of $\Delta$. Indeed, by Markov's inequality:
	\[1 - \Pd_{\mu,p}(\mathcal{G}(\Delta)) \leq n\sum_{t=0}^n \Ed_{\mu,p}(\Pd_{T_t,X_t,p}(\eta_\Delta\leq n)).\]
	Now by the Markov property, for $0\leq t\leq n$
	\[\Ed_{\mu,p}(\Pd_{T_t,X_t,p}(\eta_\Delta\leq n)) = \Pd_{\mu,p}(\exists t\leq s\leq t+n\,:\,d_{T_s}(X_s)\geq \Delta)\leq \Pd_{\mu,p}(\eta_\Delta\leq 2n).\]
	So 
	\[1 - \Pd_{\mu,p}(\mathcal{G})\leq  n\,\Pd_{\mu,p}(\eta_\Delta\leq 2n)\leq n\,\sum_{t=0}^{2n}\Pd_{\mu,p}(d_t(X_t)\geq \Delta)\leq C\,n\,(2n+D)\,e^{-\alpha\,\Delta}.\]
	Taking \[\Delta:= \left\lceil \frac{\log(2n+D) +5\log n + \log C}{\alpha}\right\rceil\]
	guarantees $\Pd_{\mu,p}(\mathcal{G}(\Delta))\geq 1 -n ^{-4}$. Plugging this choice of $\Delta$ into (\ref{eq:withoutcondition}) gives (\ref{eq:estimateescapefinite}) inside the event $\mathcal{G}(\Delta)$.\end{proof}

}
\subsection{Forgetfulness of empirical measures}\label{sec:proof.forget}

We prove here Lemma \ref{lem:forget}.

\begin{proof}[Proof of Lemma \ref{lem:forget}] The main job in the proof will be to prove the following Claim. 

\begin{claim}Let $\epsilon\in(0,1)$ be given, $\psi:\sT_*\to\R$ be $r$-local and bounded and $\mu$ be a $p$-escapable measure. Consider a trajectory $(T_t,X_t)_{t\geq 0}$ of BGRW starting from $\mu$, with empirical measures~$\widehat{P}_n$. Consider also a trajectory $(T^*_t,X_t^*)_{t\geq 0}$ of BGRW started from one end of a semi-infinite path \[T^*_0 = \{x_0=X^*_0,x_1,x_2,\dots\},\] with empirical measures $\widehat{P}^*_n$. One can couple these two processes so that: 
\[\Pd\left(\lim_{n\to +\infty}|(\widehat{P}_n - \widehat{P}^*_n)\psi|=0\right)\geq 1-\epsilon.\]\end{claim}

With this claim, one sees that, given a deterministic $c\in\R$,
\[\Pd_{\mu,p}(\widehat{P}_n\psi\to c) = 1\Leftrightarrow \Pd_{(T^*_0,x_0),p}(\widehat{P}^*_n\psi\to c) = 1.\]
This holds for {\em any} $p$-escapable measure $\mu$. In particular, if $\nu$ is {\em also} $p$-escapable $\widehat{P}_n\psi\to c$ $\Pd_{\nu,p}$-a.s., the same must hold with $\mu$ replacing $\nu$. In other words, the Claim implies the Lemma. 

Let us now prove the Claim. Take an $\ell\in\N$. Consider a chain started from measure $\nu$. Since~$\nu$ is $p$-escapable, $\tau_\ell<+\infty$ $\Pd_{\nu,p}$-almost-surely. 

Let $v_0=X_{\tau_\ell}$, $v_1$, $\dots$, $v_{\ell}$ be the unique vertices at distances $0,1,2,\dots,\ell$ at time $\tau_\ell$. Define a random time $\tau'_{\ell,r}$ as follows:
\[\tau'_{\ell,r}:=\inf\{t\geq 0\,:\,X_{\tau_\ell + t} = v_{\ell-r}\}.\]
Notice that this time may well be infinite. In fact, since ${\rm dist}(X_{\tau_\ell},v_{\ell-r})=\ell-r$, the second statement in Lemma \ref{lemma:returntime}, combined with the strong Markov property and the $p$-escapability of $\mu$, implies.  
\[\Pd_{\mu,p}\left(\tau'_{\ell,r}<+\infty\right)\leq C\,e^{-\beta\,(\ell-r)}.\] 
Note that $\tau_\ell$ is the time $X_t$ is at the tip of a path of length $\ell$ and $\tau_\ell+\tau'_{\ell,r}$ is the first time at which $X_t$ comes within distance $r$ of the other end of that path.  

Now consider the process $(T^*_t,X^*_t)$ started on vertex $x_0$ of the infinite path $x_0,x_1,\dots,x_m,\dots$. Let 
\[\tau^*_{\ell,r}:=\inf\{t\geq 0\,:\,X^*_{t} = x_{\ell-r}\}.\]
This time may also be infinite. It is easy to see that one can couple $(T^*_t,X^*_t)$ to $(T_{\tau_\ell+t},X_{\tau_\ell+t})$ so that $\tau_{\ell,r}=\tau'_{\ell,r}$ and $[T^*_t,X^*_t]_r = [T_{\tau_\ell+t},X_{\tau_\ell+t}]_r$ for all $0\leq t\leq \tau'_{\ell,r}$. Under this coupling, if~$\tau'_{\ell,r}=+\infty$, then 
\begin{eqnarray*}\widehat{P}_n\psi  &=& \frac{1}{n+1}\sum_{i=0}^n\psi(T_i,X_i) \\ \mbox{(use coupling)} &=&  \frac{1}{n+1}\sum_{i=0}^{\tau_\ell-1}\psi(X_i,T_i) +  \frac{1}{n+1}\sum_{t=0}^{n-\tau_{\ell}}\psi(T^*_{t},X^*_{t}) \\ & =&   \widehat{P}^*_n\psi + \frac{1}{n+1}\sum_{i=0}^{\tau_\ell-1}(\psi(T_i,X_i) - \psi(T_{n-\tau_\ell+i+1},X_{n-\tau_{\ell}+i+1})).\end{eqnarray*}
Since $\tau_{\ell}<+\infty$ is bounded, this implies that, under the coupling:
\[\tau'_{\ell,r}=+\infty\Rightarrow |\widehat{P}_n\psi - \widehat{P}^*_n\psi|\leq \frac{2\|\psi\|_{\infty}\,\tau_{\ell}}{n}\to 0.\]
So 
\[\Pd\left(\lim_{n\to +\infty}|(\widehat{P}_n - \widehat{P}^*_n)\psi|=0\right)\geq\Pd(\tau'_{\ell,r}=+\infty)\geq  1- C\,e^{-\beta\,(\ell-r)}.\]
In particular, this can be made $\geq 1-\epsilon$ with an appropriate choice of $\ell$.\end{proof}

